LLM4Vis: Explainable Visualization Recommendation using ChatGPT

Data visualization is a powerful tool for exploring and communicating insights in various domains. To automate visualization choice for datasets, a task known as visualization recommendation has been proposed. Various machine-learning-based approaches have been developed for this purpose, but they often require a large corpus of dataset-visualization pairs for training and lack natural explanations for their results. To address this research gap, we propose LLM4Vis, a novel ChatGPT-based prompting approach to perform visualization recommendation and return human-like explanations using very few demonstration examples. Our approach involves feature description, demonstration example selection, explanation generation, demonstration example construction, and inference steps. To obtain demonstration examples with high-quality explanations, we propose a new explanation generation bootstrapping to iteratively refine generated explanations by considering the previous generation and template-based hint. Evaluations on the VizML dataset show that LLM4Vis outperforms or performs similarly to supervised learning models like Random Forest, Decision Tree, and MLP in both few-shot and zero-shot settings. The qualitative evaluation also shows the effectiveness of explanations generated by LLM4Vis. We make our code publicly available at \href{https://github.com/demoleiwang/LLM4Vis}{https://github.com/demoleiwang/LLM4Vis}.

==> 3_background.tex <==
\section{Background: In-Context Learning}
% \yong{If we do not have enough space, the background can be removed or included in the supplementary materials.}
LLMs show a strong ability for in-context learning, enabling LLMs to effectively adapt to and solve downstream tasks using a few examples during inference without additional training~\cite{gpt3, opt, chowdhery2022palm}. 
The definition of in-context learning for text classification, as presented in~\cite{dong2022survey}, involves a frozen large language model $\mathcal{P}_{\mathrm{lm}}$ that is conditioned on in-context demonstrations $C$ to predict a suitable class $y$ for a given input text $x$, chosen from a set of candidate answers $\mathcal{Y}$.
In-context demonstrations consist of $K$ demonstrations, where each demonstration contains an input text $x_k$, a ground truth answer $y_k \in \mathcal{Y}$, and a task instruction $I_k$.
To calculate the likelihood of a candidate answer $y_i$ for the given input text $x$, a scoring function $f$ based on the entire input sequence and the frozen large language model $\mathcal{P}_{\mathrm{lm}}$ is employed, as shown in the following equation:
\begin{equation}
P(y_i | x) = f_{\mathcal{P}_{\mathrm{lm}}}(y_i, C, x).
\end{equation}
Finally, the predicted class $\hat{y}$ is determined by selecting the candidate answer with the highest score:
\begin{equation}
\hat y = \arg\max_{y_i \in \mathcal{Y}} P(y_i | x).
\end{equation}

In our approach, we designate the large language model as ChatGPT and utilize a prompt to enable ChatGPT to output the top two visualization choices directly rather than engaging in the process of ranking the score of each answer candidate. 
% \subsection{In-Context Learning for Visualization Design Choices}
% This section formulates in-context learning for visualization design choices.

==> tables/prompt_design.tex <==
\begin{table*}[t]\centering
%\footnotesize
\caption{}
% \small
\begin{tabular}{lp{13cm}}\toprule
Prompting Objective & Trigger Prompting Sentences \\ 

\midrule

Role Playing & You are a visualization recommender tasked with selecting appropriate visualization types to represent tabular data. Recommend the best visualization labels from line charts, scatter plots, bar charts, and box plots, using your knowledge of data visualization and the given rules and features of the data. \\ \hline

Visualization Recommendation & The following features correspond to the provided tabular data: ``\{\}''.
Please suggest the best visualization type for the provided features extracted from the given tabular data, and recommend labels like line charts, scatter plots, bar charts, and box plots. 
Provide the recommended visualization type in this format: `Recommended visualization type: [Type]. Recommendation rule: [Rule].' \\ \hline

Rule Generation & The provided tabular data has a ground truth recommendation of ``\{\}'', but your recommendations are incorrect. Your recommended visualization types was ``\{\}''. To improve your recommendations for future samples, please create a concise rule that uses a suitable number of features and their corresponding values from the given tabular data. Your rule must not violate any existing rules. Please provide your recommended rule in this format: `Recommendation rule: [Rule]\n' \\ \hline 

Formatting & So the rule is: ``...'' (Please ensure that the rule remains concise while retaining its original meaning). \\


\bottomrule
\end{tabular}

\label{tab:prompt_design}

\end{table*}
